Towards Context-Aware Neural Performance-Score Synchronisation

Music can be represented in multiple forms, such as in the audio form as a recording of a performance, in the symbolic form as a computer readable score, or in the image form as a scan of the sheet music. Music synchronisation provides a way to navigate among multiple representations of music in a unified manner by generating an accurate mapping between them, lending itself applicable to a myriad of domains like music education, performance analysis, automatic accompaniment and music editing. Traditional synchronisation methods compute alignment using knowledge-driven and stochastic approaches, typically employing handcrafted features. These methods are often unable to generalise well to different instruments, acoustic environments and recording conditions, and normally assume complete structural agreement between the performances and the scores. This PhD furthers the development of performance-score synchronisation research by proposing data-driven, context-aware alignment approaches, on three fronts: Firstly, I replace the handcrafted features by employing a metric learning based approach that is adaptable to different acoustic settings and performs well in data-scarce conditions. Secondly, I address the handling of structural differences between the performances and scores, which is a common limitation of standard alignment methods. Finally, I eschew the reliance on both feature engineering and dynamic programming, and propose a completely data-driven synchronisation method that computes alignments using a neural framework, whilst also being robust to structural differences between the performances and scores.

==> chapters/background.tex <==
This chapter introduces the reader to some concepts which are recurrently referenced in the thesis. We introduce Dynamic Time Warping, a prominent method used for alignment in different domains. We then briefly describe some techniques to optimize the training and performance of neural networks, which we utilize / plan to utilize in our further research.
\section{Dynamic Time Warping and its variants}\label{ssec:dtw}
Originally proposed by \cite{sakoe1978dynamic}, dynamic time warping (DTW) is a general method for finding an optimal alignment between two time series. It has been applied to various tasks like speech recognition, gesture recognition, handwriting recognition, as well as music processing. 
DTW generates an alignment between two sequences $A$= $(a_1,a_2,...,a_m)$ and $B$ = $(b_1,b_2,...,b_n)$ by comparing them using a local cost function, at each point, with the goal of minimizing the overall cost. The path which yields this minimum overall cost is then the optimal alignment between the two sequences. Formally, it can be represented as follows:

\begin{equation}
D(i, j)  = d(i, j) + min\begin{cases}
D(i, j-1) \\ D(i-1, j) \\  D(i-1,  j-1)
\end{cases}
\end{equation}
where $d(i, j)$ is the distance measure (local cost) between points $a_i$ and $b_j$; and $D(i, j)$ is the total cost for the path which generates the optimal alignment between the sequences $A_{1..i}$ and $B_{1..j}$. The local cost can be either Euclidean distance, Manhattan distance or any other function as per choice and suitability.
\begin{comment}
DTW generates a model for aligning two sequences X = (x1,x2,...,xm) and Y = (y1,y2,...,yn) by comparing them pointwise. Generally this is done by comparing the feature sequences using a local cost function, at each point, with the goal of minimizing the overall cost. The path which yields to this minimum overall cost is then the optimal alignment between the two sequences. Formally, it can be represented as follows:
\begin{equation}
D(i, j) = d(i, j) + min[D(i, j-1), D(i-1, j), D(i-1,  j-1)]
\end{equation}
where d(i, j) is the distance between points i and j (this distance can be Euclidean, Manhattan or any other of choice), and D(i, j) is the total cost for the path which generates the optimal alignment between the sequences.
\end{comment}
A possible alignment between two time-series generated using DTW is graphically illustrated in Figure \ref{dtw}.
\begin{figure}[H]
\begin{center}
\includegraphics[width=5in]{pngs/dtw1.png}
\caption{Alignment of two time-series}
\label{dtw}
\end{center}
\end{figure}

\par Multiple variants to DTW have proposed over the years, in order to improve multiple facets of the algorithm; including speed, memory complexity and modelling musical structure / adapting to the task it is being applied to. 
The introduction to DTW has been kept concise for the sake of brevity. We refer the reader to \cite{muller2015fundamentals} for a more detailed overview of DTW.

\begin{comment}
\section{Neural Networks for Music Information Processing}\label{ssec:deepmip}

\begin{figure}[H]
\begin{center}
\includegraphics[width=7in]{pngs/dnn.png}
\caption{A fully connected neural network}
\label{fcnn}
\end{center}
\end{figure}
\end{comment}



==> chapters/end_prev.tex <==
\begin{comment}
\section{Challenges to DNN based end-to-end alignment}
\begin{figure}[H]
\begin{center}
\includegraphics[width=5in]{pngs/encdec.png}
\caption{A general encoder-decoder sequence to sequence architecture}
\label{encdec2}
\end{center}
\end{figure}
End-to-end alignment involves modeling the two input sequences (audio and score) and generating an output alignment sequence (corresponding mappings). Sequence-to-sequence models \cite{sutskever2014sequence} are a natural choice for this task. A general architecture for such a model is shown in Figure \ref{encdec}, where $X_1$, $X_2$, .., $X_T$ denotes the input sequence; $C$ denotes the hidden representation and $Y_1$, $Y_2$, .., $Y_T$ denotes the output (target) sequence.


\begin{figure}[H]
\begin{center}
\includegraphics[width=5in]{pngs/RNN-longtermdependencies.png}
\label{longterm2}
\caption{RNNs typically struggle to handle long-term dependencies}
\end{center}
\end{figure}
RNNs are a standard choice for sequence to sequence models, since they are capable of incorporating temporal information. However, this capability is limited and they struggle with long input sequences, where there is presence of long-term dependencies, as depicted in Figure \label{longterm}. The reason for this is that the optimization of neural networks becomes difficult when computational graphs are too deep. This is what happens when RNNs apply the same operation repetitively at each time step for a long sequence. This results in gradients propagating over many stages, which leads to either a vanishing or exploding gradient, which impedes training and thus modeling of long sequences. We aim to overcome this barrier and develop a model which can generate robust end-to-end alignments in further stages of the PhD. We propose some methods to achieve this in the subsequent sections.


\section{Introduction}
The purpose of this report is to come up with an optimal architecture and input/output representation for end-to-end Audio-to-Score alignment. We will briefly discuss related approaches to the same and their limitations, followed by the proposed methods and different input/output representations. 

\section{Related Work}
The closest to our work is the paper on score following using reinforcement learning \cite{dorfer2018learning2}. There are certain limitations of this approach which we would like to avoid - for instance, this approach does not employ a sequential framework, and is only trained on pairs of images and audio snippets, and drastic jumps are controlled using a threshold on the speed of the score follower. Recent papers from ISMIR 2019 on alignment were aimed at bootleg score representations \cite{tanprasert2020midi} and  cross document measure-alignment \cite{waloschek2019identification}. The contemporary works are summarized in Table \ref{tab:works} for the sake of brevity.   
 \begin{table}[ht]
   \caption{A comparison of contemporary approaches to alignment}
   %\centering
   \begin{tabular}{ c c c c  c } \toprule
       \textbf{Method} & \textbf{Architecture}  & \textbf{End to end?} & \textbf{Modalities}& \textbf{Monotonic?}   \\ \midrule
        \cite{dorfer2017learning}   & Convolutional + DTW &   No   &   Image, Audio & Yes  \\ \midrule
        \cite{dorfer2018learning2}  & Convolutional &  Yes  &  Image, Audio  & Yes\\ \midrule
        \cite{tanprasert2019midi}   & Custom+DTW & No  &  Cross-modal  & Yes\\ \midrule
        \cite{waloschek2019identification}  & CNN+ResNet & No  &  Image & NA \\ \midrule
       ICASSP submission  & Siamese CNN+DTW & No  & Audio & Yes \\ \midrule
       Proposed method   & TBD  & Yes  &   Audio & No\\ \midrule
      \bottomrule
\end{tabular}
\label{tab:works2}
\end{table}   
It should be noted that \cite{waloschek2019identification} generates a coarse alignment at the measure-level across different pieces.
Works on alignment in the speech domain generally focus on forced alignment to align speech utterances with the phonemes \cite{kelley2018comparison}. 
It should be noted that \cite{waloschek2019identification} generates a coarse alignment at the measure-level across different pieces.
Works on alignment in the speech domain generally focus on forced alignment to align speech utterances with the phonemes \cite{kelley2018comparison}.
\section{Datasests}
We have the following datasets at our disposal for our experiments on end-to-end alignment. These are given in Table \ref{tab:datasets}.
\begin{table}[ht]
   \caption{Datasets used for our experiments}
   \centering
   \begin{tabular}{ c c c } \toprule
      \textbf{Name} & \textbf{Contents} & \textbf{Recordings}  \\ \midrule
      MAPS \cite{emiya2010maps} &  MIDI-audio pairs  &  238\\ \midrule
      Saarland \cite{muller2011saarland} & MIDI-audio pairs  & 50   \\ \midrule
      Mazurka \cite{sapp2007comparative} & Beat level annotations & 239 \\ \midrule
      Maestro \cite{hawthorne2018enabling} & MIDI-audio pairs & 1282 \\ \midrule
      \bottomrule
\end{tabular}
\label{tab:datasets}
\end{table} 

In addition to the aforementioned datasets, we could also employ the Tido dataset for experiments, however it needs to be confirmed with Tido if it is possible to do so. It should also be noted that the MAPS, Saarland and the Maestro dataset consist MIDI-audio pairs created using Yamaha Disklaviers, and hence are inherently aligned to a reasonable extent. Access and permission for a large dataset like that of Tido which contains original scores and performance audios with some variations thus becomes important to train robust deep models.
%\section{Proposed Methods}
%Briefly explain proposed methods and make a table if possible.
%\cite{dogan2018neural} neural multi-sequence alignment framework.

 
\subsection{Architectures}
We would like to create our own architecture by combining different types of layers suitable for the alignment task. The architecture would depend on the choice of the input-output representation, for instance, if we model it as a seq2seq problem or otherwise. We briefly highlight the major architectures with their pros, cons and computational complexities below.

1) Convolutional Layers (CNNs):

Pros:	Faster to train than RNNs, good at detecting patterns.

Cons:	Cannot capture temporality inherently.

2)	Recurrent Layers (RNNs):

Pros:	Can capture temporailty quite well until a certain sequence length.

Cons:	Vanishing gradient, slow to train since current timestep depends on previous timestep computation.

3)  Self-Attention Layers (Transformers):

Pros: Since it does not have recurrence, it can model long-term dependencies in theory. It also supports parallelization well since the representations are not computed in a sequential manner. 

Cons: If the input sequence length is too high, it can cause memory issues from a practical point of view. 

The Transformer model \cite{vaswani2017attention} is a promising network architecture and has been applied in MIR for music generation
\cite{huang2018music}.
A complexity comparison of the architectures is given below, where $n$ is the length of the sequence, $d$ is the dimension of the representation, and $k$ is the kernel size.

\begin{table}[H]
   \caption{Complexity comparison for different architectures}
   \centering
   \begin{tabular}{ c c c c} \toprule
      \textbf{Layer Type} & \textbf{Complexity per Layer} & \textbf{Sequential Operations} & \textbf{Max Path Length} \\ \midrule
      Convolutional  & O(k * n * d^2)  & O(1) & O(\log_k n) \\ \midrule
      Recurrent & O(n * d^2) & O(n)  & O(n)  \\ \midrule
      Self-Attention & O(n^2 * d)  & O(1) & O(1)  \\ \midrule
      \bottomrule
\end{tabular}
\label{results}
\end{table} 
\end{comment}
\begin{figure*}[th]
  \centering
  \includesvg[width=5.6in]{svgs/m1.svg}
  \caption{Proposed representation as a seq2seq task}
  \label{fig:meth1}
\end{figure*}
\subsection{Input-output representations}
The input-output representations could be both sequences, thereby making the alignment task a seq2seq task. 
We could also view alignment as a classification or prediction task. All the three methods are described below.


\begin{figure*}[th]
  \centering
  \includesvg[width=5.6in]{svgs/m2.svg}
  \caption{Proposed representation as a prediction task (sequence to index)}
  \label{fig:meth2}
\end{figure*}
\begin{itemize}
    \item As a sequence to sequence task
    
Proposed input-output representations:
1)	Spectrograms as inputs, Pairs of timesteps which align with each other as the output. The input size can be extended windows, generated by exploiting score information, as shown in Figure \ref{fig:meth1}.
2)	Spectrograms as inputs, and an aligned sequence as output, which preserves the type of information, and hence is easier for the model to learn. This can be, for instance, elements of the first spectral sequence at the positions of the second sequence. 
    \item As a classification task

An alternative method would be to treat the alignment task as a ternary classification task for each pair of frames, since if we consider a monotonic alignment, there are only three possible directions for the current pointer to advance, either along X, along Y or diagonally (where X and Y are the two input sequences). Thus the three classes here would determine the direction in which the pointers advance. Note that the next input pair to be considered then needs to be updated based on previous output / pointer action, hence there is higher chance of error propagation in this method.  
    \item As a prediction task
    
This is the method I am inclined to employ.	The inputs could be sliding windows (say spanning 10 seconds), and the model is trained to generate the alignment for the center
frame of the first window at each time step. The output would be the index in the second input window which aligns with the central frame of the first window. The output at each timestep is thus a single number, simplifying learning and reducing error propagation since at each timestep the input sliding windows are shifted by a fixed small amount, say one frame. The catch here would be to use a large enough window (in addition to ensuring that both audios start together rather than one audio having, say, a long silence in the beginning). We could also employ positional encodings to aid learning. This method is illustrated in Figure \ref{fig:meth2}. 

\end{itemize} 


==> chapters/publications.tex <==
\chapter*{List of publications}
\label{publications}
%The following articles have been published during this PhD:
\begin{itemize}
    \item \textbf{A Hybrid Approach to Audio-to-Score Alignment}\\ Ruchit Agrawal and Simon Dixon \\ Published at International Conference on Machine Learning (ICML 2019) in the Machine Learning for Music Discovery Workshop
    \item \textbf{Learning Frame Similarity using Siamese networks for Audio-to-Score Alignment}\\ Ruchit Agrawal and Simon Dixon \\ Published at 28th European Signal Processing Conference (EUSIPCO 2020)
    \item \textbf{Structure-Aware Audio-to-Score Alignment using Progressively Dilated Convolutional Neural Networks}\\ Ruchit Agrawal, Daniel Wolff and Simon Dixon \\ Published at IEEE International Conference on Acoustics, Speech, and Signal Processing (ICASSP 2021), 
    \item \textbf{Cross-modal performance-score synchronization using a convolutional-attentional neural network}\\ Ruchit Agrawal, Daniel Wolff and Simon Dixon \\ Under review at IEEE Signal Processing Letters (IEEE SPL)
\end{itemize}
